Deep Metric Learning-Based Out-of-Distribution Detection with Synthetic Outlier Exposure

In this paper, we present a novel approach that combines deep metric learning and synthetic data generation using diffusion models for out-of-distribution (OOD) detection. One popular approach for OOD detection is outlier exposure, where models are trained using a mixture of in-distribution (ID) samples and ``seen" OOD samples. For the OOD samples, the model is trained to minimize the KL divergence between the output probability and the uniform distribution while correctly classifying the in-distribution (ID) data. In this paper, we propose a label-mixup approach to generate synthetic OOD data using Denoising Diffusion Probabilistic Models (DDPMs). Additionally, we explore recent advancements in metric learning to train our models. In the experiments, we found that metric learning-based loss functions perform better than the softmax. Furthermore, the baseline models (including softmax, and metric learning) show a significant improvement when trained with the generated OOD data. Our approach outperforms strong baselines in conventional OOD detection metrics.

==> table.tex <==
% %%%%% Results
% \begin{table*}[ht]
%     \centering
%     \begin{adjustbox}{width=\textwidth}
%     \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
%     \hline
%      Method & \multicolumn{9}{c}{Out-of-Distribution Datasets} \\
%      \cline{2-10}

%      %%% Before outlier exposure
%      & CIFAR-100 & Tin (c) & Tin (R) & LSUN (C) & LSUN (R) & iSun & SVHN & Gaussian Noise & Uniform Noise \\
%     \hline
%      Softmax & 0.92491/0.92755/0.90586 & 0.94508/0.95450/0.92693 & 0.94508/0.95450/0.92693 & 0.97194/0.97837/0.96310 & 0.96084/0.96996/0.94735 & 0.95966/0.97130/0.93979 & 0.97641/0.96286/0.98799 & 0.83042/0.90109/0.68205 & 0.79627/0.88473/0.64203\\
%      \hline
%      Scaled Cosine (ours) & 0.78924/0.77363/0.75317 & 0.91350/0.92427/0.84860 & 0.91350/0.92427/0.84860 & 0.92598/0.92301/0.88019 & 0.91982/0.92430/0.85934 & 0.91347/0.92366/0.84034 & 0.90159/0.79551/0.92627 & 0.99018/0.99501/0.95571 & 0.98730/0.99353/0.94572\\
%      AdaCos (ours) & 0.88524/0.86837/0.88379 & 0.87367/0.86656/0.87560 & 0.87367/0.86656/0.87560 & 0.96877/0.96630/0.97030 & 0.93619/0.93242/0.93593 & 0.91918/0.91879/0.91362 & 0.97722/0.94931/0.99064 & 0.99963/0.99980/0.99811 & 1.00000/1.00000/1.00000\\
%      ArcFace (ours) &  0.87567/0.86347/0.87524 & 0.94547/0.95019/0.94104 & 0.91048/0.91897/0.89910 & 0.97103/0.97121/0.97115 & 0.94437/0.95105/0.93718 & 0.93933/0.95039/0.92516 & 0.97203/0.94372/0.98778 & 0.99930/0.99965/0.99498  & 0.99941/0.99970/0.99652\\
%      SphereFace (ours) & \\
%      CosFace (ours) & \\
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Baseline results}
%     \label{tab:results}
% \end{table*}


% %%%%% Results
% \begin{table*}[ht]
%     \centering
%     \begin{adjustbox}{width=\textwidth}
%     \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
%     \hline
%      Method & \multicolumn{9}{c}{Out-of-Distribution Datasets} \\
%      \cline{2-10}

%      %%% With outlier exposure
%      \toprule
%     Softmax (ours) & 0.91509/0.91527/0.89486 & 0.97265/0.97805/0.96684 & 0.97100/0.97578/0.96637 & 0.97416/0.97940/0.96838 & 0.98420/0.98646/0.98266  & 0.98012/0.98505/0.97470 & 0.96546/0.94795/0.98077  & 0.80807/0.88589/0.65923 & 0.91905/0.95424/0.80467\\
%      \hline
%      Scaled Cosine \cite{techapanurak2020hyperparameter} & 0.89437/0.89048/0.89186 & 0.98662/0.98711/0.98644 & 0.98662/0.98711/0.98644 & 0.97753/0.97855/0.97613 & 0.98670/0.98494/0.98828 & 0.98640/0.98762/0.9854 & 0.98346/0.96981/0.99143 & 1.00000/1.00000/1.00000 & 1.00000/1.00000/1.00000\\
%      %%%% 
%      AdaCos (ours) & 0.90270/0.90770/0.88794 & 0.96904/0.97394/0.96593 & 0.96248/0.96730/0.95898 & 0.97579/0.97853/0.97450 & 0.97661/0.97944/0.97516 & 0.97225/0.97770/0.96719 & 0.96732/0.93577/0.98625 & 0.99761/0.99878/0.98662 & 0.99775/0.99884/0.98743\\

%      %%%%%%
%      ArcFace (ours) & 0.90079/0.90014/0.88757 & 0.95819/0.96475/0.95140 & 0.95127/0.95646/0.94401 & 0.96984/0.97370/0.96706 & 0.97060/0.97538/0.96601 & 0.96526/0.97372/0.95505 & 0.96568/0.93484/0.98468 & 0.99833/0.99914/0.99090 & 0.99849/0.99921/0.9917\\
%      SphereFace (ours) & 0.90051/0.89081/0.89063 & 0.96166/0.96914/0.95533 & 0.95623/0.96416/0.94937 & 0.96933/0.97482/0.96545 & 0.97333/0.97737/0.97069 & 0.96540/0.97370/0.95639 & 0.97019/0.95010/0.98613 & 0.98918/0.99429/0.95643 & 0.98717/0.99328/0.94839\\
%      CosFace (ours) & 0.88885/0.87057/0.88301 & 0.96452/0.96939/0.96043 & 0.96067/0.96314/0.95763 & 0.97354/0.97608/0.97205  & 0.97769/0.98058/0.97624 & 0.97173/0.97792/0.96567 & 0.96939/0.94553/0.98601 & 0.99394/0.99645/0.97833 & 0.99658/0.99805/0.98514\\     
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Results after outlier exposure.}
%     \label{tab:results}
% \end{table*}




%------------------ Baseline results ------------------
\begin{table*}
  \centering
  \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{l|c|c|c|c|c|c}
      \hline
      Method & Softmax & Scaled Cosine (ours) & AdaCos (ours) & ArcFace (ours) & CosFace (ours) & SphereFace (ours)\\
      \hline
      CIFAR-100 & 0.92490/0.924754/0.90585 & 0.86936/0.87101/0.86774 & 0.88523/0.86834/0.88380 & 0.87831/0.85825/0.87844 & 0.84401/0.80550/0.85597 & 0.87363/0.85107/0.87854\\
      LSUN (C) & 0.97209/0.97836/0.96335 & 0.97652/0.97661/0.97753 & 0.96859/0.96524/0.97026 & 0.96599/0.96318/0.96685 & 0.96453/0.95992/0.96787 & 0.97366/0.97294/0.97499\\
      LSUN (R) & 0.96295/0.97171/0.95051 & 0.96085/0.96251/0.96111 & 0.94228/0.93930/0.94200 & 0.93732/0.93121/0.93869 & 0.94338/0.94470/0.94248 & 0.94106/0.93510/0.94598\\
      Tin (C) & 0.95968/0.96905/0.94492 & 0.96462/0.96772/0.96250 & 0.92802/0.92847/0.92734 & 0.91232/0.89799/0.92037 & 0.93058/0.92144/0.93380 & 0.93416/0.92913/0.93785\\
      Tin (R) & 0.94756/0.95728/0.93009 & 0.94502/0.94975/0.94208 & 0.88022/0.87244/0.88333 & 0.85841/0.83263/0.87338  & 0.89541/0.88538/0.89590 & 0.88647/0.87400/0.89563\\
      iSun & 0.96131/0.97242/0.94244 & 0.95593/0.96124/0.95192 & 0.92493/0.92456/0.91984 & 0.91876/0.91508/0.91704  & 0.93978/0.94586/0.93150 & 0.93390/0.93521/0.93219\\
      SVHN & 0.97637/0.96351/0.98790 & 0.96633/0.92955/0.98618 & 0.97849/0.95072/0.99124 & 0.96824/0.94314/0.98557 & 0.95141/0.85274/0.98212 & 0.96828/0.94721/0.98544\\
      Gaussian Noise & \textcolor{red}{0.83050/0.90114/0.68214} & 1.00000/1.00000/1.00000 & 0.99963/0.99980/0.99807 & 0.99944/0.99971/0.99661  & 1.00000/1.00000/1.00000 & 0.99942/0.99968/0.99691\\
      Uniform Noise & \textcolor{red}{0.79630/0.88476/0.64205} & 0.99999/0.99999/0.99999 & 1.00000/1.00000/1.00000 & 0.99941/0.99969/0.99627 & 1.00000/1.00000/1.00000 & 0.99972/0.99984/0.99824\\
      \hline
    \end{tabular}
  \end{adjustbox}
  \caption{Baseline results}
  \label{tab:baseline_results}
\end{table*}




\begin{table*}
  \centering
  \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{l|c|c|c|c|c|c}
      \hline
      Method & Softmax & Scaled Cosine (ours) & AdaCos (ours) & ArcFace (ours) & CosFace (ours) & SphereFace (ours)\\
      \hline
      CIFAR-100 & 0.91944/0.91937/0.90231 &  0.93351/0.93452/0.92861 & 0.89355/0.88522/0.88268 & 0.90166/0.89523/0.89118 & 0.90172/0.90568/0.89095 & 0.88835/0.88486/0.87944\\
      LSUN (C) & 0.97524/0.98039/0.96959 & 0.98336/0.98486/0.98237 & 0.97232/0.97478/0.97070 & 0.97552/0.97777/0.97426 & 0.97364/0.97572/0.97283 & 0.96911/0.97169/0.96769\\
      LSUN (R) & 0.98411/0.98641/0.98256 & 0.99020/0.99087/0.98995 & 0.97764/0.98111/0.97519 & 0.98133/0.98393/0.97960 & 0.97212/0.97544/0.96992 & 0.97277/0.97475/0.97171\\
      Tin (C) & 0.97377/0.97929/0.96791 & 0.98474/0.98674/0.98313 & 0.95464/0.96008/0.94841 & 0.96719/0.97336/0.96194 & 0.96068/0.96614/0.95655 & 0.94425/0.94507/0.94192\\
      Tin (R) & 0.97257/0.97693/0.96832 & 0.98379/0.98538/0.98283 & 0.95289/0.95649/0.94756 & 0.96489/0.96938/0.96018 & 0.95166/0.95793/0.94662 & 0.93528/0.93289/0.93528\\
      iSun & 0.98048/0.98499/0.97541 & 0.98846/0.99041/0.98662 & 0.96816/0.97604/0.95976 & 0.97362/0.97972/0.96701 & 0.96498/0.97237/0.95752 & 0.96216/0.96776/0.95660\\
      SVHN & 0.96173/0.94292/0.97837 & 0.98536/0.97350/0.99296 & 0.96387/0.93633/0.98337 & 0.97900/0.95722/0.99117 & 0.96849/0.94414/0.98571 & 0.97565/0.95354/0.98948\\
      Gaussian Noise & 0.97594/0.98510/0.95055 & 0.99983/0.99991/0.99901 & 0.99981/0.99988/0.99968 & 0.99929/0.99960/0.99612 & 0.99917/0.99956/0.99540 & 0.99944/0.99968/0.99691\\
      Uniform Noise & 0.98540/0.99111/0.96767 & 0.99990/0.99995/0.99912 & 0.99992/0.99994/0.99990 & 0.99948/0.99974/0.99623 & 0.99984/0.99990/0.99972 & 0.99942/0.99967/0.99695\\
      \hline
    \end{tabular}
  \end{adjustbox}
  \caption{Results with outlier exposure.}
  \label{tab:outlier_exposure}
\end{table*}



